Exploring Test-time Scaling via Prediction Merging on Large-Scale Recommendation

Inspired by the success of language models (LM), scaling up deep learning recommendation systems (DLRS) has become a recent trend in the community. All previous methods tend to scale up the model parameters during training time. However, how to efficiently utilize and scale up computational resources during test time remains underexplored, which can prove to be a scaling-efficient approach and bring orthogonal improvements in LM domains. The key point in applying test-time scaling to DLRS lies in effectively generating diverse yet meaningful outputs for the same instance. We propose two ways: One is to explore the heterogeneity of different model architectures. The other is to utilize the randomness of model initialization under a homogeneous architecture. The evaluation is conducted across eight models, including both classic and SOTA models, on three benchmarks. Sufficient evidence proves the effectiveness of both solutions. We further prove that under the same inference budget, test-time scaling can outperform parameter scaling. Our test-time scaling can also be seamlessly accelerated with the increase in parallel servers when deployed online, without affecting the inference time on the user side. Code is available.

==> tables/Param_vs_Pred_table.tex <==
\begin{table*}[!htbp]
    \renewcommand\arraystretch{1.15}
    \centering
    \caption{Performance Comparison: Model Merging (Model) vs. Prediction Merging (Pred).}
    \label{table:merging}
    \vspace{-5pt}
    \resizebox{1.0\textwidth}{!}{
    \begin{tabular}{c|c|cc|cc|cc|cc|cc|cc|cc|cc}
        \hline
                                                & \multirow{2}{*}{Method} & \multicolumn{2}{c|}{FNN} & \multicolumn{2}{c|}{IPNN} & \multicolumn{2}{c|}{DeepFM} & \multicolumn{2}{c|}{DCN} & \multicolumn{2}{c|}{DCNv2} & \multicolumn{2}{c|}{FinalMLP} & \multicolumn{2}{c|}{Wukong} & \multicolumn{2}{c}{RankMixer} \\
        \cline{3-18}                            &                         & AUC$\uparrow$           & LogLoss$\downarrow$            & AUC$\uparrow$               & LogLoss$\downarrow$           & AUC$\uparrow$              & LogLoss$\downarrow$                & AUC$\uparrow$               & LogLoss$\downarrow$                & AUC$\uparrow$ & LogLoss$\downarrow$      & AUC$\uparrow$ & LogLoss$\downarrow$      & AUC$\uparrow$ & LogLoss$\downarrow$      & AUC$\uparrow$ & LogLoss$\downarrow$ \\
        \hline
        \multirow{10}{*}{\rotatebox{90}{Avazu}} & Backbone-Model          & 0.7885                  & 0.3764                    & 0.7914                      & 0.3743                   & 0.7869                     & 0.3757                        & 0.7882                      & 0.3766                        & 0.7944        & 0.3712              & 0.7858        & 0.3777              & 0.7954        & 0.3705              & 0.7952        & 0.3706         \\
        \cline{2-18}
                                                & 2$\times$-Model         & 0.6856                  & 0.5279                    & 0.7003                      & 0.5415                   & 0.7757                     & 0.5545                        & 0.7095                      & 0.5204                        & 0.7707        & 0.5302              & 0.7681        & 0.5446              & 0.7152        & 0.6586              & 0.7689        & 0.6195         \\
                                                & 2$\times$-Pred          & 0.7895                  & 0.3757                    & 0.7926                      & 0.3733                   & 0.7871                     & 0.3755                        & 0.7896                      & 0.3754                        & 0.7952        & 0.3707              & 0.7882        & 0.3758              & 0.7972        & 0.3694              & 0.7962        & 0.3699         \\
        \cline{2-18}
                                                & 4$\times$-Model         & 0.5748                  & 0.6260                    & 0.5871                      & 0.6263                   & 0.7463                     & 0.6384                        & 0.7081                      & 0.6076                        & 0.7447        & 0.6303              & 0.6377        & 0.6105              & 0.6942        & 0.6790              & 0.7289        & 0.6725         \\
                                                & 4$\times$-Pred          & 0.7903                  & 0.3748                    & 0.7934                      & 0.3728                   & 0.7873                     & 0.3754                        & 0.7903                      & 0.3749                        & 0.7956        & 0.3704              & 0.7892        & 0.3744              & 0.7986        & 0.3685              & 0.7971        & 0.3793         \\
        \cline{2-18}
                                                & 8$\times$-Model         & 0.5215                  & 0.6679                    & 0.4930                      & 0.6569                   & 0.7003                     & 0.6604                        & 0.7103                      & 0.6575                        & 0.7412        & 0.6686              & 0.5876        & 0.6300              & 0.5778        & 0.6831              & 0.6756        & 0.6819         \\
                                                & 8$\times$-Pred          & 0.7906                  & 0.3747                    & 0.7938                      & 0.3725                   & 0.7873                     & 0.3754                        & 0.7906                      & 0.3747                        & 0.7958        & 0.3703              & 0.7898        & 0.3741              & 0.7994        & 0.3681              & 0.7981        & 0.3689         \\
        \cline{2-18}
                                                & 16$\times$-Model        & 0.5102                  & 0.6899                    & 0.5179                      & 0.6723                   & 0.6713                     & 0.6677                        & 0.7036                      & 0.6879                        & 0.7343        & 0.6832              & 0.5304        & 0.6483              & 0.4941        & 0.6847              & 0.4924        & 0.6829         \\
                                                & 16$\times$-Pred         & \textbf{0.7907}         & \textbf{0.3746}           & \textbf{0.7940}             & \textbf{0.3723}          & \textbf{0.7873}            & \textbf{0.3754}               & \textbf{0.7908}             & \textbf{0.3745}               & \textbf{0.7959} & \textbf{0.3702}   & \textbf{0.7904} & \textbf{0.3737}   & \textbf{0.8001} & \textbf{0.3676}   & \textbf{0.7988} & \textbf{0.3684} \\
        \hline
        \multirow{10}{*}{\rotatebox{90}{Criteo}} & Backbone-Model         & 0.8103                  & 0.4411                    & 0.8109                      & 0.4405                   & 0.8102                     & 0.4413                        & 0.8103                      & 0.4412                        & 0.8116        & 0.4399              & 0.8105        & 0.4410              & 0.8103        & 0.4411              & 0.8115        & 0.4400         \\
        \cline{2-18}
                                                & 2$\times$-Model         & 0.7848                  & 0.6135                    & 0.7873                      & 0.6332                   & 0.7582                     & 0.5751                        & 0.7822                      & 0.5897                        & 0.7704        & 0.5480              & 0.7796        & 0.6071              & 0.7571        & 0.6507              & 0.7741        & 0.6387         \\
                                                & 2$\times$-Pred          & 0.8110                  & 0.4405                    & 0.8117                      & 0.4397                   & 0.8112                     & 0.4404                        & 0.8110                      & 0.4405                        & 0.8124        & 0.4391              & 0.8112        & 0.4404              & 0.8121        & 0.4395              & 0.8130        & 0.4386         \\
        \cline{2-18}
                                                & 4$\times$-Model         & 0.7350                  & 0.6675                    & 0.7533                      & 0.6717                   & 0.6664                     & 0.5966                        & 0.7512                      & 0.6533                        & 0.7472        & 0.6240              & 0.7405        & 0.6571              & 0.7066        & 0.6831              & 0.7242        & 0.6645         \\
                                                & 4$\times$-Pred          & 0.8113                  & 0.4402                    & 0.8122                      & 0.4393                   & 0.8116                     & 0.4400                        & 0.8114                      & 0.4401                        & 0.8129        & 0.4387              & 0.8116        & 0.4400              & 0.8131        & 0.4387              & 0.8138        & 0.4379         \\
        \cline{2-18}
                                                & 8$\times$-Model         & 0.6210                  & 0.6838                    & 0.6646                      & 0.6889                   & 0.6538                     & 0.6008                        & 0.7527                      & 0.6771                        & 0.7387        & 0.6599              & 0.5923        & 0.6721              & 0.6679        & 0.6825              & 0.7024        & 0.6685         \\
                                                & 8$\times$-Pred          & 0.8115                  & 0.4400                    & 0.8123                      & 0.4391                   & 0.8118                     & 0.4399                        & 0.8115                      & 0.4400                        & 0.8130        & 0.4385              & 0.8117        & 0.4398              & 0.8135        & 0.4383              & 0.8141        & 0.4376         \\
        \cline{2-18}
                                                & 16$\times$-Model        & 0.5000                  & 0.6901                    & 0.4998                      & 0.6946                   & 0.6531                     & 0.6042                        & 0.7540                      & 0.6899                        & 0.7254        & 0.6788              & 0.5000        & 0.6754              & 0.6109        & 0.6830              & 0.6812        & 0.6682         \\
                                                & 16$\times$-Pred         & \textbf{0.8115}         & \textbf{0.4399}           & \textbf{0.8124}             & \textbf{0.4390}          & \textbf{0.8119}            & \textbf{0.4397}               & \textbf{0.8116}             & \textbf{0.4399}               & \textbf{0.8132} & \textbf{0.4384}   & \textbf{0.8118} & \textbf{0.4398}   & \textbf{0.8137} & \textbf{0.4381}   & \textbf{0.8143} & \textbf{0.4374} \\
        \hline
        \multirow{10}{*}{\rotatebox{90}{KDD12}}  & Backbone-Model         & 0.8108                  & 0.1500                    & 0.8118                      & 0.1498                   & 0.8086                     & 0.1505                        & 0.8106                      & 0.1501                        & 0.8114        & 0.1499              & 0.8111        & 0.1499              & 0.8116        & 0.1498              & 0.8124        & 0.1496         \\                                
        \cline{2-18}
                                                & 2$\times$-Model         & 0.7574                  & 0.5436                    & 0.7169                      & 0.5330                   & 0.7480                     & 0.2451                        & 0.7609                      & 0.3405                        & 0.7635        & 0.3857              & 0.7385        & 0.4647              & 0.6826        & 0.6186              & 0.7497        & 0.6014         \\
                                                & 2$\times$-Pred          & 0.8114                  & 0.1499                    & 0.8127                      & 0.1496                   & 0.8099                     & 0.1502                        & 0.8113                      & 0.1499                        & 0.8118        & 0.1497              & 0.8116        & 0.1498              & 0.8128        & 0.1496              & 0.8132        & 0.1494         \\
        \cline{2-18}
                                                & 4$\times$-Model         & 0.6022                  & 0.5636                    & 0.6027                      & 0.5488                   & 0.7369                     & 0.3662                        & 0.7499                      & 0.4906                        & 0.7140        & 0.5388              & 0.5961        & 0.4806              & 0.5931        & 0.6478              & 0.6583        & 0.6410         \\
                                                & 4$\times$-Pred          & 0.8116                  & 0.1498                    & 0.8131                      & 0.1495                   & 0.8106                     & 0.1500                        & 0.8115                      & 0.1499                        & 0.8122        & 0.1497              & 0.8120        & 0.1497              & 0.8133        & 0.1495              & 0.8139        & 0.1493         \\
        \cline{2-18}
                                                & 8$\times$-Model         & 0.4988                  & 0.5637                    & 0.5321                      & 0.5519                   & 0.7422                     & 0.4376                        & 0.7550                      & 0.5785                        & 0.6912        & 0.6242              & 0.5002        & 0.4857              & 0.5694        & 0.6538              & 0.4880        & 0.6439         \\
                                                & 8$\times$-Pred          & 0.8118                  & 0.1498                    & 0.8133                      & 0.1494                   & 0.8110                     & 0.1499                        & 0.8117                      & 0.1498                        & 0.8123        & 0.1496              & 0.8122        & 0.1497              & 0.8135        & 0.1494              & 0.8144        & 0.1491         \\
        \cline{2-18}
                                                & 16$\times$-Model        & 0.4992                  & 0.5661                    & 0.5027                      & 0.5525                   & 0.7360                     & 0.5053                        & 0.7503                      & 0.6295                        & 0.6934        & 0.6535              & 0.5000        & 0.4824              & 0.6273        & 0.6538              & 0.4859        & 0.6447         \\
                                                & 16$\times$-Pred         & \textbf{0.8119}         & \textbf{0.1498}           & \textbf{0.8134}             & \textbf{0.1494}          & \textbf{0.8112}            & \textbf{0.1499}               & \textbf{0.8118}             & \textbf{0.1498}               & \textbf{0.8124} & \textbf{0.1496}   & \textbf{0.8122} & \textbf{0.1497}   & \textbf{0.8137} & \textbf{0.1494}   & \textbf{0.8148} & \textbf{0.1491} \\
        \hline
    \end{tabular}
    }
    
    \begin{tablenotes}
        \footnotesize 
        \item[1] \textbf{Model} denotes model weight merging (averaging parameters from models trained with different seeds), while \textbf{Pred} denotes prediction merging (averaging outputs over different seeds).  Model merging performance degrades significantly as the number of merged models increases, demonstrating that directly merging model weights does not work for CTR models. In contrast, prediction merging consistently improves performance with more seeds, showing that CTR models are more nuanced than typical LMs where weight averaging is effective. \textbf{Bold} font indicates the best results at 16× scale.
        \vspace{-10pt}
    \end{tablenotes}
\end{table*}

